Transition magnetic moments for $\Delta \rightarrow p$ transition in asymmetric nuclear matter

In the present work we calculate the transition magnetic moments for the radiative decays of $\Delta$ baryon to proton $(\Delta \rightarrow p)$ in isospin asymmetric nuclear medium at finite temperature using chiral SU(3) quark mean field model. Within the framework of chiral SU(3) mean field model, the properties of baryons in asymmetric medium are modified through the exchange of scalar fields $(\sigma, \zeta, \delta)$ and vector fields $(\omega, \rho)$. The isospin asymmetry of medium is taken into account via scalar-isovector field $\delta$ and vector iso-vector field $\rho$. We calculate the in-medium masses of quarks, proton and $\Delta$ baryon in asymmetric matter within the chiral SU(3) quark mean field model and use these as input in the chiral constituent quark ($\chi$CQM) model to calculate the in-medium transition magnetic moments for $(\Delta \rightarrow p)$ transition for different values of isospin asymmetry of hot and dense medium. For calculating the magnetic moments of baryons, contributions of valence quarks, quark sea and orbital angular momentum of quark sea are considered in these calculations.

==> Ref.tex <==
@article{hayano2010hadron, 
	
	author={Hayano, Ryugo S and Hatsuda, Tetsuo},
	journal={Rev. Mod. Phys.},
	volume={$\textbf{82}$},
	
	pages={2949},
	year={2010},
	publisher={APS}
}




@article{Holzenkamp:1989tq,
	author = "Holzenkamp, B. and Holinde, K. and Speth, J.",
	_title = "{A Meson Exchange Model for the Hyperon Nucleon Interaction}",
    journal = "Nucl. Phys. A",
	volume = {$\textbf{500}$},
	pages = 485,
	year = "1989"
}
@article{Haidenbauer:2018gvg,
	author = "Haidenbauer, J. and Mei\ss{}ner, U. -G.",
	_title = "{In-medium properties of a $\Xi N$ interaction derived from chiral effective field theory}",
    journal = "Eur. Phys. J. A",
	volume = {$\textbf{55}$},
	pages = "23",
	year = "2019"
}
@article{Tolos:2020aln,
	author = "Tolos, Laura and Fabbietti, Laura",
	_title = "{Strangeness in Nuclei and Neutron Stars}",
	
	journal = "Prog. Part. Nucl. Phys.",
	volume = {$\textbf{112}$},
	pages = "103770",
	year = "2020"
}

@article{Rafelski:2000by,
	author = "Rafelski, Johann and Letessier, Jean",
	_title = "{Sudden hadronization in relativistic nuclear collisions}",
	
	journal = "Phys. Rev. Lett.",
	volume ={$\textbf{85}$},
	pages = "4695",
	year = "2000"
}
@article{Pushkina:2004wa,
	author = "Pushkina, Irina and  \textit{et al.}",
	collaboration = "QCD-TARO",
	_title = "{Properties of hadron screening masses at finite baryonic density}",

	journal = "Phys. Lett. B",
	volume = {$\textbf{609}$},
	pages = "265",
	year = "2005"
}



@article{Knospe:2017oin,
	author = "Knospe, A. G.",
	editor = "Mischke, A. and Kuijer, P.",
	_title = "{Resonance Production in Heavy-Ion Collisions}",
	journal = "EPJ Web Conf.",
	volume = {$\textbf{171}$},
	pages = "09001",
	year = "2018"
}


%%%%%%%%%%%

@article{Harrison:2003sb,
author = "Harrison, M. and Ludlam, T. and Ozaki, S.",

journal = "Nucl. Instrum. Meth. A",
volume = {$\textbf{499}$},
pages = "235",
year = "2003"
}
@article{friman2011cbm,
	author={Friman, Bengt and \textit{et al.}},
	journal={Lect. Notes Phys.},
	volume={$\textbf{814}$},
	year={2011},
	publisher={Springer}
}
@article{kumar2013star,
	
	author={Kumar, Lokesh and \textit{et al.}},
	journal={Nucl. Phys.  A},
	volume={$\textbf{904}$},
	pages={256c},
	year={2013},
	publisher={Elsevier}
}

@article{odyniec2010rhic,
	
	author={Odyniec, Grazyna},
	journal={J. Phys. G: Nucl. Part. Phys.},
	volume={$\textbf{37}$},
	pages={094028},
	year={2010},
	publisher={IOP Publishing}
}
@article{evans2007large,
	author={Evans, Lyndon},
	journal={New J. Phys.},
	volume={$\textbf{9}$},
	pages={335},
	year={2007},
	publisher={IOP Publishing}
}
@article{DiNezza:2024ctw,
	author = "Di Nezza, P. and \textit{et al.}",
	journal = "PoS",
	volume={$\textbf{SPIN2023}$},
	pages = "036",
	year = "2024"
}
@article{Odyniec:2019kfh,
	author = "Odyniec, Grazyna",
	journal = "PoS",
	volume={$\textbf{CORFU2018}$},
	pages = "151",
	year = "2019"
}  
@article{Liu:2022cqh,
	author = "Liu, C. and others",
	journal = "Phys. Rev. Accel. Beams",
	volume={$\textbf{25}$},
	
	pages = "051001",
	year = "2022"
}
@article{Liu:2022wme,
	author = "Liu, Chuyu and others",
	journal = "JACoW",
	volume={$\textbf{IPAC2022}$},
	pages = "1908",
	year = "2022"
}


@article{senger2012compressed,
	
	author={Senger, Peter},
	journal={Cent. Eur. J. Phys.},
	volume={$\textbf{10}$},
	pages={1289},
	year={2012},
	publisher={Versita}
}
@article{rapp2010charmonium,
	
	author={Rapp, R and \textit{et al.}},
	journal={Prog. Part. Nucl. Phys. },
	volume={$\textbf{65}$},
	
	pages={209},
	year={2010},
	publisher={Elsevier}
}
@article{Sawada:2007gy,
	author = "Sawada, S.",
	journal = "Nucl. Phys. A",
	volume={$\textbf{782}$},
	pages = "434",
	year = "2007"
}
@article{Hotchi:2017krx,
	author = "Hotchi, H. and others",
	
	journal = "Phys. Rev. Accel. Beams",
	volume={$\textbf{20}$},
	
	pages = "060402",
	year = "2017"
}
@article{Kekelidze:2017ghu,
	author = "Kekelidze, V. D. and  \textit{et al.}",
	journal = "Phys. Part. Nucl.",
	volume={$\textbf{48}$},
	pages = "727",
	year = "2017"
}

@article{Kekelidze:2017tgp,
	author = "Kekelidze, V. D. and \textit{et al.}",
	journal = "Nucl. Phys. A",
	volume={$\textbf{967}$},
	pages = "8847",
	year = "2017"}
	
@article{EuropeanMuon:1983wih,
     author = "Aubert, J. J. and others",
     collaboration = "European Muon",
     _title = "{The ratio of the nucleon structure functions $F2_n$ for iron and deuterium}",
    _reportNumber = "CERN-EP/83-14",
    _doi = "10.1016/0370-2693(83)90437-9",
     journal = "Phys. Lett. B",
     volume = "{\bf 123}",
     pages = "275",
     year = "1983"
 }
 
 
 @article{He:2004kg,
     author = "He, Jun and Dong, Yu-Bing",
     _title = "{Magnetic moments and electromagnetic radii of nucleon and Delta(1232) in an extended GBE model}",
     _eprint = "nucl-th/0404011",
     _archivePrefix = "arXiv",
     _doi = "10.1088/0253-6102/43/1/027",
     journal = "Commun. Theor. Phys.",
     volume = "{$\textbf{43}$}",
     pages = "139",
     year = "2005"
 }
 
 
 @article{Faessler:2006ft,
     author = "Faessler, Amand and Gutsche, Th. and Ivanov, M. A. and Korner, J. G. and Lyubovitskij, V. E. and Nicmorus, D. and Pumsa-ard, K.",
     _title = "{Magnetic moments of heavy baryons in the relativistic three-quark model}",
     _eprint = "hep-ph/0602193",
     _archivePrefix = "arXiv",
     _doi = "10.1103/PhysRevD.73.094013",
     journal = "Phys. Rev. D",
     volume = "{$\textbf{73}$}",
     pages = "094013",
     year = "2006"
 }
 
 @article{Schlumpf:1993rm,
     author = "Schlumpf, Felix",
     _title = "{Magnetic moments of the baryon decuplet in a relativistic quark model}",
     _eprint = "hep-ph/9305293",
     _archivePrefix = "arXiv",
     _reportNumber = "SLAC-PUB-6218",
     _doi = "10.1103/PhysRevD.48.4478",
     journal = "Phys. Rev. D",
     volume = "{$\textbf{48}$}",
     pages = "4478",
     year = "1993"
 }
 
 
 
 @article{Lee:1997jk,
     author = "Lee, Frank X.",
     _title = "{Determination of decuplet baryon magnetic moments from QCD sum rules}",
     _eprint = "hep-ph/9708323",
     _archivePrefix = "arXiv",
     _reportNumber = "CU-NPL-1152",
     _doi = "10.1103/PhysRevD.57.1801",
     journal = "Phys. Rev. D",
     volume = "$\textbf{57}$",
     pages = "1801",
     year = "1998"
 }
 
 @article{Aliev:2008ay,
     author = "Aliev, T. M. and Azizi, K. and Ozpineci, A.",
     _title = "{Magnetic Moments of Heavy $\Xi_{Q}$ Baryons in Light Cone QCD Sum Rules}",
     _eprint = "0803.4420",
     _archivePrefix = "arXiv",
     _primaryClass = "hep-ph",
     _doi = "10.1103/PhysRevD.77.114006",
     journal = "Phys. Rev. D",
     volume = "{$\textbf{77}$}",
     pages = "114006",
     year = "2008"
 }
 
 @article{Aliev:2000cy,
     author = "Aliev, T. M. and Ozpineci, A.",
     _title = "{Magnetic moments of decuplet baryons in light cone QCD}",
     _eprint = "hep-ph/0003304",
     _archivePrefix = "arXiv",
     _doi = "10.1103/PhysRevD.62.053012",
     journal = "Phys. Rev. D",
     volume = "$\textbf{62}$",
     pages = "053012",
     year = "2000"
 }
 
 @article{Ledwig:2008es,
     author = "Ledwig, Tim and Silva, Antonio and Vanderhaeghen, Marc",
     _title = "{Electromagnetic properties of the Delta(1232) and decuplet baryons in the self-consistent SU(3) chiral quark-soliton model}",
     _eprint = "0811.3086",
     _archivePrefix = "arXiv",
     _primaryClass = "hep-ph",
     _doi = "10.1103/PhysRevD.79.094025",
     journal = "Phys. Rev. D",
     volume = "$\textbf{79}$",
     pages = "094025",
     year = "2009"
 }
 
 @article{Li:2016ezv,
     author = "Li, Hao-Song and Liu, Zhan-Wei and Chen, Xiao-Lin and Deng, Wei-Zhen and Zhu, Shi-Lin",
     _title = "{Magnetic moments and electromagnetic form factors of the decuplet baryons in chiral perturbation theory}",
     _eprint = "1608.04617",
     _archivePrefix = "arXiv",
     _primaryClass = "hep-ph",
     _reportNumber = "ADP-16-31-T986",
     _doi = "10.1103/PhysRevD.95.076001",
     journal = "Phys. Rev. D",
     volume = "$\textbf{95}$",
     _number = "7",
     pages = "076001",
     year = "2017"
 }
 
 
 @article{Ryu:2008st,
     author = "Ryu, C. Y. and Hyun, C. H. and Park, T. -S. and Hong, S. W.",
     _title = "{Magnetic moment of hyperons in dense matter}",
     _eprint = "0806.1099",
     _archivePrefix = "arXiv",
     _primaryClass = "nucl-th",
     _doi = "10.1016/j.physletb.2009.02.049",
     journal = "Phys. Lett. B",
     volume = "$\textbf{674}$",
     pages = "122",
     year = "2009"
 }
 
 @article{Ryu:2010tr,
     author = "Ryu, C. Y. and Hyun, C. H. and Cheoun, Myung-Ki",
     _title = "{Magnetic moments of octet baryons at finite density and temperature}",
     _eprint = "1008.2051",
     _archivePrefix = "arXiv",
     _primaryClass = "nucl-th",
     _doi = "10.1088/0954-3899/37/10/105002",
     journal = "J. Phys. G",
     volume = "$\textbf{37}$",
     pages = "105002",
     year = "2010"
 }
 
 @article{Ramalho:2012pu,
     author = "Ramalho, G. and Tsushima, K. and Thomas, A. W.",
     _title = "{Octet Baryon Electromagnetic form Factors in Nuclear Medium}",
     _eprint = "1206.2207",
     _archivePrefix = "arXiv",
     _primaryClass = "hep-ph",
     _reportNumber = "ADP-12-25-T792",
     _doi = "10.1088/0954-3899/40/1/015102",
     journal = "J. Phys. G",
     volume = "$\textbf{40}$",
     pages = "015102",
     year = "2013"
 }
 
 @article{Arifi:2024tix,
     author = "Arifi, Ahmad Jafar and Hutauruk, Parada T. P. and Tsushima, Kazuo",
     _title = "{In-medium electromagnetic form factors of pseudoscalar mesons from the quark model}",
     eprint = "2412.09883",
     archivePrefix = "~arXiv",
     primaryClass = "hep-ph",
     _reportNumber = "LFTC-24-11/94",
     _month = "12",
     _year = "2024"
}
 

@article{Dutt:2024lui,
    author = "Dutt, Suneel and Kumar, Arvind and Dahiya, Harleen",
    _title = "{Effective masses and magnetic moments of charmed baryons in asymmetric hot strange hadronic matter}",
    _eprint = "2409.11878",
    _archivePrefix = "arXiv",
    _primaryClass = "hep-ph",
    _doi = "10.1103/PhysRevD.110.116003",
    journal = "Phys. Rev. D",
    volume = "$\textbf{110}$",
    _number = "11",
    pages = "116003",
    year = "2024"}
    
@article{Singh:2016hiw,
    author = "Singh, Harpreet and Kumar, Arvind and Dahiya, Harleen",
    _title = "{Magnetic Moments of Octet Baryons in Hot and Dense Nuclear Matter}",
    _eprint = "1608.03388",
    _archivePrefix = "arXiv",
    _primaryClass = "hep-ph",
    _doi = "10.1088/1674-1137/41/9/094104",
    journal = "Chin. Phys. C",
    volume = "$\textbf{41}$",
    _number = "9",
    pages = "094104",
    year = "2017"
} 

@article{Singh:2017mxj,
    author = "Singh, Harpreet and Kumar, Arvind and Dahiya, Harleen",
    _title = "{Octet Baryon Masses and Magnetic Moments in Hot and Dense Isospin Asymmetric Nuclear Matter}",
    _eprint = "1710.08328",
    _archivePrefix = "arXiv",
    _primaryClass = "nucl-th",
    _doi = "10.1140/epjp/i2019-12486-4",
    journal = "Eur. Phys. J. Plus",
    volume = "$\textbf{134}$",
    _number = "3",
    pages = "128",
    year = "2019"
} 
 
 @article{Singh:2020nwp,
     author = "Singh, Harpreet and Kumar, Arvind and Dahiya, Harleen",
     _title = "{Decuplet baryons in nuclear and hyperonic medium}",
     _doi ="10.1140/epjp/s13360-020-00397-6",
     journal = "Eur. Phys. J. Plus",
     volume = "$\textbf{135}$",
     _number = "6",
     pages = "422",
     year = "2020"
 }
 
 
 @article{Kumar:2023owb,
     author = "Kumar, Arvind and Dutt, Suneel and Dahiya, Harleen",
     _title = "{Magnetic moments of decuplet baryons in asymmetric strange hadronic matter at finite temperature}",
     _eprint = "2311.02936",
     _archivePrefix = "arXiv",
     _primaryClass = "nucl-th",
     _doi ="10.1140/epja/s10050-023-01228-9",
     journal = "Eur. Phys. J. A",
     volume = "$\textbf{60}$",
     _number = "1",
     pages = "4",
     year = "2024"
 }
  
}@article{Dutt:2024lui,
    author = "Dutt, Suneel and Kumar, Arvind and Dahiya, Harleen",
    _title = "{Effective masses and magnetic moments of charmed baryons in asymmetric hot strange hadronic matter}",
    _eprint = "2409.11878",
    _archivePrefix = "arXiv",
    _primaryClass = "hep-ph",
    _doi = "10.1103/PhysRevD.110.116003",
    _journal = "Phys. Rev. D",
    volume = "$\textbf{110}$",
    _number = "11",
    pages = "116003",
    year = "2024"
} 
 
 
 @article{Kaur:2024wze,
     author = "Kaur, Navpreet and Puhan, Satyajit and Pandey, Reetanshu and Kumar, Arvind and Dutt, Suneel and Dahiya, Harleen",
     _title = "{Does nuclear medium affect the transverse momentum-dependent parton distributions of valence quark of pions?}",
     _eprint = "2409.05394",
     _archivePrefix = "arXiv",
     _primaryClass = "hep-ph",
     _doi = "10.1016/j.physletb.2024.139114",
     journal = "Phys. Lett. B",
     volume = "$\textbf{859}$",
     pages = "139114",
     year = "2024"
 }
 
 @article{Puhan:2024xdq,
     author = "Puhan, Satyajit and Kaur, Navpreet and Kumar, Arvind and Dutt, Suneel and Dahiya, Harleen",
     _title = "{Pion valence quark distributions in asymmetric nuclear matter at finite temperature}",
     _eprint = "2408.07334",
     _archivePrefix = "arXiv",
     _primaryClass = "nucl-th",
     _doi = "10.1103/PhysRevD.110.054042",
     journal = "Phys. Rev. D",
     volume = "$\textbf{110}$",
     _number = "5",
     pages = "054042",
     year = "2024"
 }
 
 
@article{Singh:2024lra,
    author = "Singh, Dhananjay and Puhan, Satyajit and Kaur, Navpreet and Kaur, Manpreet and Kumar, Arvind and Dutt, Suneel and Dahiya, Harleen",
    _title = "{Effect of Asymmetric Nuclear Medium on the Valence Quark Structure of the Kaons}",
    eprint = "2410.20181",
    archivePrefix = " arXiv",
    primaryClass = "hep-ph",
    _month = "10",
    _year = "2024"
}

@article{Wang:2001jw,
    author = "Wang, Ping and Zhang, Zong-Ye and Yu, You-Wen",
    _title = "{Nuclear matter in a chiral SU(3) quark mean field model}",
    journal = "Commun. Theor. Phys.",
    volume = "$\textbf{36}$",
    pages = "71",
    year = "2001"
}

@article{Wang:2005vg,
    author = "Wang, P. and Lawley, S. and Leinweber, Derek Bruce and Thomas, Anthony William and Williams, Anthony Gordon",
    _title = "{Neutron stars and strange stars in the chiral SU(3) quark mean field model}",
    _eprint = "nucl-th/0506014",
    _archivePrefix = "arXiv",
    _reportNumber = "ADP-05-12-T622, JLAB-THY-05-312",
    _doi = "10.1103/PhysRevC.72.045801",
    journal = "Phys. Rev. C",
    volume = "$\textbf{72}$",
    pages = "045801",
    year = "2005"
}

@article{Li:2017vmq,
    author = "Li, Hao-Song and Liu, Zhan-Wei and Chen, Xiao-Lin and Deng, Wei-Zhen and Zhu, Shi-Lin",
    _title = "{Decuplet to octet baryon transitions in chiral perturbation theory}",
    _eprint = "1706.06458",
    _archivePrefix = "arXiv",
    _primaryClass = "hep-ph",
    _doi = "10.1140/epjc/s10052-019-6592-z",
    journal = "Eur. Phys. J. C",
    volume = "$\textbf{79}$",
    _number = "1",
    pages = "66",
    year = "2019"
}

@article{Fayyazuddin:2020vpe,
    author = "Fayyazuddin and Aslam,
     M. Jamil",
    _title = "{Radiative Baryonic Decay $\mathcal{B}^{*}\left(\frac{3}{2}\right)\to\mathcal{B}\left(\frac{1}{2}\right)+\gamma$ in Constituent Quark Model: A Tutorial}",
    eprint = "2011.06750",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    _month = "11",
    _year = "2020"
}

@article{Kim:2020lgp,
    author = "Kim, June-Young and Kim, Hyun-Chul",
    _title = "{Electromagnetic transition form factors, $E2/M1$ and $C2/M1$ ratios of the baryon decuplet}",
    _eprint = "2002.05980",
    _archivePrefix = "arXiv",
    _primaryClass = "hep-ph",
    _reportNumber = "INHA-NTG-01/2020",
    _doi = "10.1140/epjc/s10052-020-08657-6",
    journal = "Eur. Phys. J. C",
    volume = "$\textbf{80}$",
    _number = "11",
    pages = "1087",
    year = "2020"
}

@article{Dahiya:2018ahb,
    author = "Dahiya, Harleen",
    _title = "{Transition magnetic moments of $J^P=\frac{3}{2}^+$ decuplet to $J^P=\frac{1}{2}^+$ octet baryons in the chiral constituent quark model}",
    _eprint = "1806.04864",
    _archivePrefix = "arXiv",
    _primaryClass = "hep-ph",
    _doi = "10.1088/1674-1137/42/9/093102",
    journal = "Chin. Phys. C",
    volume = "$\textbf{42}$",
    _number = "9",
    pages = "093102",
    year = "2018"
}



@article{Barik:2013lna,
    author = "Barik, N. and Mishra, R. N. and Mohanty, D. K. and Panda, P. K. and Frederico, T.",
    _title = "{Nuclear equation of state in a relativistic independent quark model with chiral symmetry and dependence on quark masses}",
    _eprint = "1307.0934",
    _archivePrefix = "arXiv",
    _primaryClass = "nucl-th",
    _doi = "10.1103/PhysRevC.88.015206",
    journal = "Phys. Rev. C",
    volume = "$\textbf{88}$",
    _number = "1",
    pages = "015206",
    year = "2013"
}

@article{Cheng:1994zn,
    author = "Cheng, T. P. and Li, Ling-Fong",
    _title = "{Flavor and spin contents of the nucleon in the quark model with chiral symmetry}",
    _eprint = "hep-ph/9410345",
    _archivePrefix = "arXiv",
    _reportNumber = "CMU-HEP-94-30",
    _doi = "10.1103/PhysRevLett.74.2872",
    journal = "Phys. Rev. Lett.",
    volume = "$\textbf{74}$",
    pages = "2872",
    year = "1995"
}

@article{Dahiya:2002fp,
   author = "Dahiya, Harleen and Gupta, Manmohan",
    _title = "{Octet magnetic moments and the Coleman-Glashow sum rule violation in the chiral quark model}",
    _eprint = "hep-ph/0208134",
    _archivePrefix = "arXiv",
    _doi = "10.1103/PhysRevD.66.051501",
    journal = "Phys. Rev. D",
    volume = "$\textbf{66}$",
    pages = "051501",
    year = "2002"
}

@article{Girdhar:2015gsa,
    author = "Girdhar, Aarti and Dahiya, Harleen and Randhawa, Monika",
    _title = "{Magnetic moments of $J^P=\frac{3}{2}^+$ decuplet baryons using effective quark masses in chiral constituent quark model}",
    _eprint = "1508.00308",
    _archivePrefix = "arXiv",
    _primaryClass = "hep-ph",
    _doi = "10.1103/PhysRevD.92.033012",
    journal = "Phys. Rev. D",
    volume = "$\textbf{92}$",
    _number = "3",
    pages = "033012",
    year = "2015"
}

 @article{Sharma:2010vv,
     author = "Sharma, Neetika and Dahiya, Harleen and Chatley, P. K. and Gupta, Manmohan",
     _title = "{Spin ${^1_\overline 2}^+$, spin $^{3+}_\overline 2$ and transition magnetic moments of low lying and charmed baryons}",
     _eprint = "1003.4338",
     _archivePrefix = "arXiv",
     _primaryClass = "hep-ph",
     _doi = "10.1103/PhysRevD.81.073001",
     journal = "Phys. Rev. D",
     volume = "$\textbf{81}$",
     pages = "073001",
     year = "2010"
 }
 
 @article{Dahiya:2018ahb,
     author = "Dahiya, Harleen",
     _title = "{Transition magnetic moments of $J^P=\frac{3}{2}^+$ decuplet to $J^P=\frac{1}{2}^+$ octet baryons in the chiral constituent quark model}",
     _eprint = "1806.04864",
     _archivePrefix = "arXiv",
     _primaryClass = "hep-ph",
     _doi = "10.1088/1674-1137/42/9/093102",
     journal = "Chin. Phys. C",
     volume = "$\textbf{42}$",
     _number = "9",
     pages = "093102",
     year = "2018"
 }
